Information Theoretically Secure Hypothesis Test for Temporally Unstructured Quantum Computation (Extended Abstract)

The efficient certification of classically intractable quantum devices has been a central research question for some time. However, to observe a "quantum advantage", it is believed that one does not need to build a large scale universal quantum computer, a task which has proven extremely challenging. Intermediate quantum models that are easier to implement, but which also exhibit this quantum advantage over classical computers, have been proposed. In this work, we present a certification technique for such a sub-universal quantum server which only performs commuting gates and requires very limited quantum memory. By allowing a verifying client to manipulate single qubits, we exploit properties of measurement based blind quantum computing to give them the tools to test the "quantum superiority" of the server.

==> eptcsdata.tex <==
\providecommand{\firstpage}{209}
\providecommand{\publicationstatus}{Bob Coecke and Aleks Kissinger (Eds.):\\ 14th International Conference on Quantum Physics and Logic (QPL)\\
EPTCS 266, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.266.14}{10.4204/EPTCS.266.14}}

